Learning Activation Functions to Improve Deep Neural Networks

Artificial neural networks typically have a fixed, non-linear activation function at each neuron. We have designed a novel form of piecewise linear activation function that is learned independently for each neuron using gradient descent. With this adaptive activation function, we are able to improve upon deep neural network architectures composed of static rectified linear units, achieving state-of-the-art performance on CIFAR-10 (7.51%), CIFAR-100 (30.83%), and a benchmark from high-energy physics involving Higgs boson decay modes.

==> sec-RelatedWork.tex <==
\section{Related Work}
Recently, a deep neural network called ``maxout network'' \citep{wang2013maxout} have used an activation function that takes the maximum of the output of multiple linear functions. This hidden unit can approximate any convex function. However, it cannot produce something similar to non-convex activation functions which have proven useful, such as the sigmoid and tanh units. Our method has the ability to also approximate non-convex functions, as shown in section \ref{sec:learnedfunctions}.

Previous research has modified activation functions through genetic and evolutionary algorithms \citep{yao1999evolving} \citep{turner2014neuroevolution}. These algorithms allow neural networks to have different activation functions for different neurons. However, these algorithms are known for being slow, whereas our method uses backpropagation which does not take much more computation time.
